Party Prediction for Twitter

A large number of studies on social media compare the behaviour of users from different political parties. As a basic step, they employ a predictive model for inferring their political affiliation. The accuracy of this model can change the conclusions of a downstream analysis significantly, yet the choice between different models seems to be made arbitrarily. In this paper, we provide a comprehensive survey and an empirical comparison of the current party prediction practices and propose several new approaches which are competitive with or outperform state-of-the-art methods, yet require less computational resources. Party prediction models rely on the content generated by the users (e.g., tweet texts), the relations they have (e.g., who they follow), or their activities and interactions (e.g., which tweets they like). We examine all of these and compare their signal strength for the party prediction task. This paper lets the practitioner select from a wide range of data types that all give strong performance. Finally, we conduct extensive experiments on different aspects of these methods, such as data collection speed and transfer capabilities, which can provide further insights for both applied and methodological research.

==> 202reltable_ivado_presentation.tex <==
%\newpage
%\begin{table*}[htbp]
%\begin{center}
%\begin{tabular}{ l| c | c|c|c|c|}
   %    \diagbox{Method}{Signal}    & \rotatebox{80}{content} & \rotatebox{80}{relation} & \rotatebox{80}{activity}  & \rotatebox{80}{media} & \rotatebox{80}{reported performance}\\ 
%\hline  
%	method1 &  &  &   & \CheckmarkBold &\\ 
%    method2    &  &   &  & \CheckmarkBold& \\ 
%        method3 &  &  &   & \CheckmarkBold &\\ 
%        \method &  &  &   & \CheckmarkBold &\\ \hline
%\end{tabular} 
%\caption{ {\bf \method matches all specs}, while competitors
%miss one or more of the features.\label{tab:salesman}}
%\end{center}
%\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\begin{table*}[th!]
\caption{Survey methods to predict party affiliation. Here we report for each paper:  Accuracy, whether they used Media outlets, Network Activities (retweets and mentions), Network Relation (followership), and Content  (words and  hashtags); as well as if they consider  Public, Elite or both, their test size in terms of number of users on which the ideology is inferred, if their code is available and finally the level of difficulty. %, as explained more in the text.  
}\vspace{-9pt}
\label{tab:literature_survey}
\resizebox{1\linewidth}{!}
{%
\begin{tabular}{l|c|cccc|lrc}
 
\textbf{Methods} &
%   \rotb{Accuracy (1)} &
%   \rotb{Media outlets (2)} &
%   \rotb{\begin{tabular}[c]{@{}c@{}}Network Activities\\   (retweets and mentions) (3)\end{tabular}} &
%   \rotb{\begin{tabular}[c]{@{}c@{}}Network Relation\\ (fellowship) (4)\end{tabular}} &
%   \rotb{\begin{tabular}[c]{@{}c@{}}Content \\ (words and  hashtags) (5) \end{tabular}} &
%   \rotb{Public vs. Elite} &
%   \rotb{Test size} &
%   \rotb{Code available?} &
%   \rotb{Level of Difficulty} \\ 
  \textbf{Accuracy} &
  \textbf{Media} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Activity \end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Relation \end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Content  \end{tabular}} &
  \textbf{Type} &
  \textbf{Size} & % (users)} &
  \textbf{Difficulty} \\ 
  %\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Dataset Difficulty: \\ (how many users? any filter on users?\\  type (politicians or their followers), \\ type \& amount of activity,\\  keywords they have use?)\end{tabular}}} &
  \hline
%    
\cit{conover2011predicting}%r et al. (2011) 
&
  95   &
   &
  \X &
   &
  \X &
  Public &
  1,000  &
 % \begin{tabular}[c]{@{}l@{}}* Users well-connected \\ * At least one political hashtag.\end{tabular} &
  Medium \\
  \hline
%    
\textbf{\cit{barbera2015birds},\cite{Barber2015TweetingFL}} %rá et al. (2015) 
&
  \textbf{78}   &
   &
   &
  \X &
   &
  Both &
  42,008   &
  %\begin{tabular}[c]{@{}l@{}}* Users with more than 100 tweets.\\ * 25 or more followers.\\ * Follow 100 or more. \\ * English.\\ * Mention collection keywords. \\ *(Non) Political hashtags.\end{tabular} &
  \textbf{Hard} \\
  \hline
   
\cit{rheault2021efficient}
% and Musulan (2021)
&
  91   &
  \X &
  \X &
   &
  \X &
  Politicians &
  505  &
  %\begin{tabular}[c]{@{}l@{}}* Hashtags referring to the \\ 2019 Canadian election\\ * True party affiliation\end{tabular} &
   Easy \\
   \hline
    
\cit{luceri2019red}
% i et al. (2019)
&
  89   &
  \X &
  \X &
   &
   &
  Public &
  38,000  &
  %\begin{tabular}[c]{@{}l@{}}*Other 1 million accounts labelled\\ with the retweet network of the users\end{tabular} &
  \begin{tabular}[c]{@{}c@{}} Medium \end{tabular} \\
  \hline
   
\cit{colleoni2014echo}
% ni et al. (2014) 
&
  79   &
   &
   &
  \X &
  \X &
  Public &
  10,551  &
  %\begin{tabular}[c]{@{}l@{}}* Political tweets\\ * Follow Democrat or Republican\\  accounts.\end{tabular} &
  Medium \\
  \hline
   
\cit{pennacchiotti2011machine}
% acchiotti and Popescu (2011)
&
  89   &
   &
  \X &
  \X &
  \X &
  Public &
  10,338 &
  %* Classified themselves. &
  Medium \\
  \hline
   
% Stefanov et al. (2020) 
\cit{stefanov2020predicting}
&
  83   &
  \X &
  \X &
   &
  \X&
  Public &
  806  &
  %\begin{tabular}[c]{@{}l@{}}* Discuss one of 8 eight political topics.\\ * Located in the USA.\\ * URLs from media with known bias.\end{tabular} &
  Medium \\
  \hline
   
% Gu et al. (2016)
\cit{gu2016ideology}
&
  66   &
   &
  \X &
  \X &
   &
  Both &
  1,200  &
  Medium 
 % \begin{tabular}[c]{@{}l@{}}* Users connected to a set of politicians.\\ * Followed by at least 20 politicians \\ * Follow only 3 to 5  politicians.\end{tabular} & N0
   \\
   \hline
    
% Badawy et al. (2018) 
\cit{badawy2018analyzing}&
  91   &
  \X &
  \X &
   &
   &
  Public &
  29,000 &
  %\begin{tabular}[c]{@{}l@{}}* Retweet messages from left or right media.\\ * Keywords related to U.S. Presidential election.\\ *Keywords related to D.Trump and H. Clinton.\\ *Keywords for other parties added.\end{tabular} &
  Medium \\
  \hline
   
% Xiao et al. (2020)
\cit{xiao2020timme}&
  96   &
   &
  \X &
  \X &
   &
  Both &
  20,811  &
 % \begin{tabular}[c]{@{}l@{}}* Accounts of politicians and candidates. \\ * Crawling of every tweet of each user (public).\\ * Keen on political affairs and moderate interests.\end{tabular} &
  Hard\\
  \hline
   
  \textbf{\cit{preoctiuc2017beyond}} &
  \textbf{97}   &
   &
   &
   \X &
   \X&
   Public &
   13,651  &
   \textbf{Medium} \\
   \hline
   \cit{rodriguez2022urjc}
% and Musulan (2021)
&
  82   &
   &
   &
   &
  \X &%1029600
  Politicians  &
  12,600  &
  %\begin{tabular}[c]{@{}l@{}}* Hashtags referring to the \\ 2019 Canadian election\\ * True party affiliation\end{tabular} &
   Easy \\
      \hline
% \cit{rodriguez2022urjc}
% % and Musulan (2021)
% &
%   84   &
%   &
%   &
%   &
%   \X &
%   Politicians (left) &
%   6,840  &
%   %\begin{tabular}[c]{@{}l@{}}* Hashtags referring to the \\ 2019 Canadian election\\ * True party affiliation\end{tabular} &
%   &
%   Easy \\
%       \hline
   
% \cit{rodriguez2022urjc}
% % and Musulan (2021)
% &
%   79   &
%   &
%   &
%   &
%   \X &
%   Politicians (right) &
%   5,760  &
%   %\begin{tabular}[c]{@{}l@{}}* Hashtags referring to the \\ 2019 Canadian election\\ * True party affiliation\end{tabular} &
%   &
%   Easy \\
%     \hline
   
\cit{mou2021align}
% and Musulan (2021)
&
  80   &
   &
   &
  \X &
  \X &
  Politicians &
  735  &
  %\begin{tabular}[c]{@{}l@{}}* Hashtags referring to the \\ 2019 Canadian election\\ * True party affiliation\end{tabular} &
   Easy \\
\end{tabular}}\vspace{-5pt}
\end{table*}





==> 501conclu.tex <==
%\newpage



\begin{table*}[bh!]
\caption{Appendix: Survey methods to predict ideology (with accuracy below 65\% or no mention of the accuracy) %, as explained more in the text.  
}\vspace{-5pt}
\label{tab:literature_survey_appendix}
\resizebox{.95\linewidth}{!}
{%
\begin{tabular}{l|c|cccc|lrcc}
\textbf{Methods} &
%   \rotb{Accuracy (1)} &
%   \rotb{Media outlets (2)} &
%   \rotb{\begin{tabular}[c]{@{}c@{}}Network Activities\\   (retweets and mentions) (3)\end{tabular}} &
%   \rotb{\begin{tabular}[c]{@{}c@{}}Network Relation\\ (fellowship) (4)\end{tabular}} &
%   \rotb{\begin{tabular}[c]{@{}c@{}}Content \\ (words and  hashtags) (5) \end{tabular}} &
%   \rotb{Public vs. Elite} &
%   \rotb{Test size} &
%   \rotb{Code available?} &
%   \rotb{Level of Difficulty} \\ 
  \textbf{Accuracy} &
  \textbf{Media} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Activity \end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Relation \end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Content  \end{tabular}} &
  \textbf{Type} &
  \textbf{Size} & % (users)} &
  \textbf{Code} &
  \textbf{Difficulty} \\ 
 \hline
\cit{liu2022politics} &
  <50\% &
   &
   &
   &
  \X &
  
    \begin{tabular}[c]{@{}l@{}} Public \end{tabular} &
    1,079 &
    %\href{https://github.com/launchnlp/politics}
    {\X} 
    & Hard \\
    \hline
\cit{pastor2020spotting}
&
  NA &
   &
   &
   &
  \X &
  
    \begin{tabular}[c]{@{}l@{}} Public \end{tabular} &
    20,364 &
    %\href{https://github.com/CyberDataLab/botbusters-spanish-general-elections}
    {\X} 
    & Easy \\
    \hline
\cit{sinno2022political} &
 55\% &
   \X &
   &
   &
  \X& 
  Political news &
  175 &
  &
  Easy \\
 \hline
\cit{yang2022twitter} &
   NA &
   \X &
   &
   &
  \X& 
  Public &
   NA &
  %\href{https://zenodo.org/record/6547792}
  {\X}&
  Easy
   \\
   \hline
   \cit{chen2015mass}&
   NA &
    &
   &
  \X &
  \X& 
  Both &
   NA &
  &
  Hard
   \\
   \hline
      \cit{bright2016explaining}&
   NA &
    &
   \X &
   &
  \X & 
  Both &
   NA &
   &
  Medium
   \\
   \hline
      \cit{gaisbauer2021ideological}&
   NA &
    &
   \X &
   &
  \X & 
  Both &
   NA &
   &
  Medium
   \\
   \hline
      \cit{garimella2017long} &
   NA &
   \X &
   \X &
   \X &
  \X & 
  Both &
   NA &
   &
  Medium
   \\
   \hline
    \cit{kamienski2022measuring} &
   NA &
    &
   \X &
   \X &
  \X & 
  Public &
   NA &
    &
  Easy
   \\
   \hline
\end{tabular}}\vspace{-5pt}
\end{table*}

 


==> FIG/voter_matching_stats.tex <==
\begin{table}[]
    \caption{Users matched to their voter registration. Voters* and Users* respectively correspond to the number of unique voters in the records and unique Twitter users in our data.}
    \label{tab:voter_registration_stats}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|llllll}
        State                & Voters* & Users* & Matched & Democrat & Republican & Other \\ \hline
        Ohio                 & 7,771,590     & 4,913          &  1,431    & 320 & 193 & 917    \\
        New York             & 17,718,437    & 30,927             & 8,255  & 4,843 & 1,631 & 1,781       \\
        Florida              & 14,477,882    & 50,541             & 12,905  & 5,585 & 4,508 & 2,810      \\
        Arkansas             & 1,722,465     & 4,311              & 1,280   & 145 & 140 & 995      \\
        District of Columbia & 510,026       & 17,661             & 2,538   & 1,929 & 153 & 456      \\
        North Carolina       & 8,004,814     & 20,761             & 6,050    & 2,450 & 1,655 & 1,945  \\
        \hline
        Total & & & 32,456 & 15,272 & 8,280 & 8,904\\
        \hline
    \end{tabular}
    }
\end{table}
